Confidence Boosts Trust-Based Resilience in Cooperative Multi-Robot Systems

Wireless communication-based multi-robot systems open the door to cyberattacks that can disrupt safety and performance of collaborative robots. The physical channel supporting inter-robot communication offers an attractive opportunity to decouple the detection of malicious robots from task-relevant data exchange between legitimate robots. Yet, trustworthiness indications coming from physical channels are uncertain and must be handled with this in mind. In this paper, we propose a resilient protocol for multi-robot operation wherein a parameter {\lambda}t accounts for how confident a robot is about the legitimacy of nearby robots that the physical channel indicates. Analytical results prove that our protocol achieves resilient coordination with arbitrarily many malicious robots under mild assumptions. Tuning {\lambda}t allows a designer to trade between near-optimal inter-robot coordination and quick task execution; see Fig. 1. This is a fundamental performance tradeoff and must be carefully evaluated based on the task at hand. The effectiveness of our approach is numerically verified with experiments involving platoons of autonomous cars where some vehicles are maliciously spoofed.

==> Sections/deviation-legitimate-old.tex <==
%!TEX ROOT = ../resilient_consensus_trust.tex

\subsubsection{Deviation due to Legitimate Agents}
Before proceeding with the deviation bound for the legitimate contribution,
we state ancillary results used in the proof.

\begin{lemma}[Difference of positive matrices]\label{lem:matrix-difference-general}
	Let $\ell > 0$ and $X,Y\in\Real{N\times N}$ be two positive matrices such that $[X]_{ii} \ge \ell$ and $[Y]_{ii} \ge \ell$ for $i = 1,\dots,N$.
	Then,
	it holds
	\begin{equation}
		[|X-Y|\one]_{i} \le [X\one]_{i} + [Y\one]_{i}-2\ell, \quad i = 1,\dots,N,
	\end{equation}
	where $|A|$ denotes the matrix with elements $|[A]_{ij}|$.
	\begin{proof}
		It is a trivial generalization of~\cite[Lemma~4]{Yemini22tro-resilienceConsensusTrust}.
	\end{proof}
\end{lemma}

\begin{cor}[Difference of sub-stochastic matrices\protect{~\cite[Lemma~4]{Yemini22tro-resilienceConsensusTrust}}]\label{lem:matrix-difference}
	Let $\ell > 0$ and $X,Y\in\Real{N\times N}$ be two sub-stochastic matrices such that $[X]_{ii} \ge \ell$ and $[Y]_{ii} \ge \ell$ for $i = 1,\dots,N$.
	Then,
	$[|X-Y|\one]_{i} \le 2(1-\ell)$ for $i = 1,\dots,N$.
\end{cor}

\begin{lemma}[Non-amplification of input]\label{lem:prod-w-substochastic}
	Let $\{\lam{t}\}_{t\ge0}$ be a sequence such that $\lam{t}\in[0,1] \ \forall t$.
	Then,
	for any $t_1, t_2 \in\Realp{}$,
	\begin{equation}\label{eq:prod-lam-less-1}
		\sum_{t=t_1}^{t_2}\lr\prodlam{s}{t+1}{t_2} \rr\lam{t}\le 1
	\end{equation}
	with equality if $\lam{t}\equiv1$.
	Moreover,
	the matrix
	\begin{equation}\label{eq:prod-W-substochastic}
		\sum_{t=t_1}^{t_2}\lr\prodW{s}{t+1}{t_2} \rr\lam{t}
	\end{equation}
	is sub-stochastic
	and is the identity matrix if $\lam{t}\equiv1$.
	\begin{proof}
		It follows by induction.
		See \cref{app:substochastic-sequence} for details.
	\end{proof}
\end{lemma}

We now bound the probability that~\eqref{eq:state-leg-error} exceeds a threshold at steady state.
We develop the derivation of the bound in two parts,
associated with two different components of $\statelegerr{i}{t}$.
Let
\begin{equation}\label{eq:Wt}
	\Wlegerr{t} = \Wlegerr[1]{t} + \Wlegerr[2]{t}
\end{equation}
where
\begin{equation}\label{eq:leg-err-contribution-lambda}
	\Wlegerr[1]{t} \doteq \prodW{k}{0}{t-1} - \left(\prod_{k=0}^{t-1}(1-\lambda_k) \right)\lr\Wlegtrue\rr^\infty
\end{equation}
expresses the mismatch with the nominal (true) weights and
\begin{multline}\label{eq:leg-err-contribution-misclassification}
	\Wlegerr[2]{t} \doteq \sum_{k=0}^{t-1} \lr\prodW{s}{k+1}{t-1}\rr\lam{k}\\
	-\lr1-\prodlam{k}{0}{t-1}\rr\lr\Wlegtrue\rr^\infty
\end{multline}
is associated with the input $\{\lam{t}\stateleg{0}\}_{t\ge0}$ that anchors the legitimate agents to their initial condition.

We now note that the arguments in the proof of \cref{prop:consensus} can be used to show that both $\statelegerr{i}{t}$ and the two deviation terms respectively associated with $\Wlegerr[1]{t}$ and $\Wlegerr[2]{t}$ converge to a consensus under the event $\tf<\infty$.
Hence,
using the same argument in~\eqref{eq:limsup-prob-partition}--\eqref{eq:lim} with $\statelegerr{i}{t}$ in place of $\stateerr{i}{t}$ and applying the triangle and Markov's inequalities,
it follows that\footnote{We omit the conditioning event $\tf<\infty$ according to our convention.}
\begin{multline}\label{eq:leg-err-markov-limit}
	\pr{\lim_{t\rightarrow\infty}\statelegerr{i}{t} > \epsilon} \le \dfrac{1}{\epsilon} \mean{\lim_{t\rightarrow\infty}\left| \ls \Wlegerr[1]{t}\stateleg{0}\rs_i \right|} +\\ \dfrac{1}{\epsilon}\mean{\lim_{t\rightarrow\infty}\left| \ls \Wlegerr[2]{t}\stateleg{0}\rs_i \right|}.
\end{multline}
We next use~\eqref{eq:leg-err-markov-limit} to retrieve a probabilistic bound for~\eqref{eq:state-leg-error}.

\begin{lemma}\label{lemma:deviation-leg-one}
	Let
	\begin{equation}\label{eq:s}
		s(\gamma)\doteq-\frac{1}{\gamma}-\frac{\ln(1-ce^{-\gamma})}{\gamma}\cdot \frac{1-ce^{-\gamma}}{ce^{-\gamma}}.
	\end{equation}
	Then,
	for all $i\in\leg$,
	it holds
	\begin{equation}\label{eq:deviation-leg-one-bound}
		\mean{\lim_{t\rightarrow\infty}\left| \ls \Wlegerr[1]{t}\stateleg{0}\rs_i \right|} \le \eta\uleg[1]{}
	\end{equation}
	where
	\begin{equation}
		\uleg[1]{} \doteq 2\e^{s(\gamma)}\lr1-\lr\dfrac{1}{\dmax+1}\rr^{\mean{\tf}}\rr.
	\end{equation}
	\begin{proof}
		See \cref{app:proof-deviation-leg-one}.
	\end{proof}
\end{lemma}

\cref{lemma:deviation-leg-one} bounds the deviation of a consensus-type protocol with learned weights~\eqref{eq:weights-trust} rather than with (unknown) true weights~\eqref{eq:weights-true}.
It thus expresses a ``structural'' limitations because the legitimate agents do not know who the malicious agents are.
Bound~\eqref{eq:deviation-leg-one-bound} is ruled by $s(\gamma)$ that it is an increasing function of $\gamma$.
In words,
this suggests that setting $\gamma$ small (that makes $\lam{t}$ decay slowly) is beneficial to performance because legitimate agents learn the trustworthy neighbors while also keeping the weights balanced (thus avoiding biases caused by misclassification of legitimate neighbors) during this learning process.
This is reminiscent of the strategy proposed in~\cite{Yemini22tro-resilienceConsensusTrust},
where the consensus protocol starts at $T_0$ and a larger value of $T_0$ helps to reduce the deviation term associated with data exchange among legitimate agents. %makes the agents later but with a higher confidence in the learned weights.
Moreover,
$\uleg[1]{}$ increases with $\mean{\tf}$,
suggesting that later detection yields larger deviation.

\begin{lemma}\label{lemma:deviation-leg-two}
	Let $\vmin \doteq \min_{i\in\leg}v_i$ and $\ell\doteq\min\{\ell_1,\ell_2\}$ where
	\begin{gather}
		\begin{multlined}
			\ell_1 \doteq\lr1-c\e^{-\gamma(\maxof{\tf}{1})}\rr^{\frac{1}{1-\e^{-\gamma}}} \lr c\e^{-\gamma(\maxof{(\tf-1)}{0})} \right.\\
			\left. + c\lr\dfrac{1-c\e^{-\gamma}}{\dmax+1}\rr^{\tf-1}\dfrac{1-\e^{-\gamma(\tf-1)}}{1-\e^{-\gamma}}\one[\{\tf>1\}] \rr
		\end{multlined}\label{eq:l1}\\
		\ell_2\doteq 1-\e^{s(\gamma)}.\label{eq:l2}
	\end{gather}
	Then,
	for all $i\in\leg$,
	it holds
	\begin{equation}\label{eq:deviation-leg-two-bound}
		\mean{\lim_{t\rightarrow\infty}\left| \ls \Wlegerr[2]{t}\stateleg{0}\rs_i \right|} \le \eta \uleg[2]{}
	\end{equation}
	where
	\begin{equation}\label{eq:u2}
		\uleg[2]{} \doteq 1- \prodlam{k}{0}{\infty} + \sum_{k=0}^{\infty}\lr\prodlam{s}{k+1}{\infty}\rr\lam{k} - 2\vmin\mean{\ell}.
	\end{equation}
	\begin{proof}
		See \cref{app:proof-deviation-leg-two}.
	\end{proof}
\end{lemma}

\begin{rem}[Explicit bound for input contribution]
	The bound in \cref{lem:deviation-leg} is tighter than the one in~\cite[Lemma~3]{acc},
	which uses \cref{lem:matrix-difference} instead of \cref{lem:matrix-difference-general} that considers the exact norms of sub-stochastic matrices.
	While simplifying the infinite products in~\eqref{eq:u2} is generally hard,
	the following approximation yields a nontrivial bound for large enough $\gamma$:
	\begin{equation}\label{eq:u2-appr}
		\uleg[2]{} \le 1 - \lr1-c\rr^{\frac{1}{1-\e^{-\gamma}}} + c\dfrac{c\e^{-\gamma} - \e^{-\gamma} - 1}{\e^{-2\gamma} - 1} - 2\vmin\mean{\ell}.
	\end{equation}
\end{rem}

\marginnote{Do we want to remove this proposition and jump to \cref{thm:bound}?}
\begin{prop}\label{lem:deviation-leg}
	The deviation from nominal consensus due to the contribution by legitimate agents can be bounded as
	\begin{equation}\label{eq:leg-err-prob-bound}
		\mean{\lim_{t\rightarrow\infty}\statelegerr{i}{t}} \le \eta(\uleg[1]{} + \uleg[2]{}), \quad \forall i\in\leg.
	\end{equation}
%	where
%	\begin{equation}\label{eq:leg-bound-prob}
%		\uleg{} \doteq \uleg[1]{} + \uleg[2]{}}.
%	\end{equation}
	\begin{proof}
		Applying the triangle inequality to~\eqref{eq:Wt} and assuming that the limits exist yields
		\begin{equation}\label{eq:Wt-tr-ineq}
			\lim_{t\rightarrow\infty}\statelegerr{i}{t} \le \lim_{t\rightarrow\infty}\left| \ls \Wlegerr[1]{t}\stateleg{0}\rs_i \right| + \lim_{t\rightarrow\infty}\left| \ls \Wlegerr[2]{t}\stateleg{0}\rs_i \right|.
		\end{equation}
		The claim follows combining~\eqref{eq:Wt-tr-ineq} with~\eqref{eq:deviation-leg-one-bound} and~\eqref{eq:deviation-leg-two-bound}.
	\end{proof}
\end{prop}

A few remarks are in order to understand bound~\eqref{eq:leg-err-prob-bound} and how it behaves as $\gamma$ varies.
The behavior of $\uleg{\epsilon}$ is mainly affected by two functions of $\gamma$,
which are $\e^{s(\gamma)}$ and $\mean{\ell}$.
%as regards dependence on $\gamma$,
%the  function  while the second is proportional to the negative expectation of $\ell$ w.r.t. $\tf$.

The second function appearing in $\uleg{\epsilon}$ is proportional to the negative expectation of $\ell$ w.r.t. $\tf$ and expresses the impact of the input term $\lam{t}\state{0}{i}$ in~\eqref{eq:update-rule-regular} that anchors the legitimate agents to their initial condition.
It is not easy to analytically evaluate the minimum $\ell=\min\{\ell_1,\ell_2\}$,
in general.
Nonetheless,
the following facts hold:
\begin{enumerate}[label=(\arabic*)]
	\item the term $\ell_2$ is strictly decreasing with $\gamma$;
	\item the term $\ell_1$ is strictly increasing with $\gamma$ for $\tf\le1$,
	while for $\tf>1$ it is the product between an increasing and a decreasing function of $\gamma$;
	\item the limits of the two terms evaluate
	\begin{subequations}
		\begin{gather}
			\ell_1^0\doteq\lim_{\gamma\rightarrow0}\ell_1 = 0\\
			\ell_2^0\doteq\lim_{\gamma\rightarrow0}\ell_2 = \vmin\\
			\ell_1^\infty\doteq\lim_{\gamma\rightarrow\infty}\ell_1 = \vmin c\one[\{\tf\le1\}]+\dfrac{\vmin c\one[\{\tf>1\}]}{\lr\dmax+1\rr^{\tf-1}}\label{eq:ell1-lim-inf}\\
			\ell_2^\infty\doteq\lim_{\gamma\rightarrow\infty}\ell_2 = c\vmin
		\end{gather}
	\end{subequations}
	and it follows
	\begin{equation}\label{eq:limits-ineq}
		\ell_1^0 < \ell_2^0, \qquad \ell_1^\infty \le \ell_2^\infty
	\end{equation}
	where the equality $\ell_1^\infty = \ell_2^\infty$ holds if and only if $\tf\le1$;
	\item from~\eqref{eq:ell1-lim-inf},
	it further follows that $\ell_1^\infty$ decreases with $\tf$ and $\lim_{\tf\rightarrow\infty}\ell_1^\infty=0$.
	%	Moreover,
	%	for $\tf>0$,
	%	we have $\ell_1^\infty > \ell_2^0$.
\end{enumerate}
From the items (1)--(3) above and continuity of $\ell_1$ and $\ell_2$,
we infer the following result,
summarized as a lemma.
\begin{lemma}\label{lem:bound-deviation}
	If $\tf\le1$,
	it holds $\ell=\ell_1$.
	If $\tf>1$,
	there exist $\bar{\gamma}_1>0$ and $\bar{\gamma}_2>0$ such that 
	%	it holds $\ell \rightarrow\ell_1^\infty$ as $\gamma\rightarrow0$ and $\ell \rightarrow \ell_2^\infty$ as $\gamma\rightarrow\infty$.
	%	Further,
	%	by continuity,
	%	\eqref{eq:limits-ineq} implies 
	$\ell=\ell_1$ for $\gamma<\bar{\gamma}_1$ and $\gamma>\bar{\gamma}_2$.
	%	for some with $\bar{\gamma}_1\le\bar{\gamma}_2$.
	%	and the lower bound is $\ell=\ell_1$ for $\gamma<\bar{\gamma}_1$ and $\ell = \ell_2$ for $\gamma>\bar{\gamma}_2$.
\end{lemma}
\cref{lem:bound-deviation} implies that,
for $\tf\le1$,
$\ell=\ell_1$ and thus the term $-\ell$ is decreasing with $\gamma$.

On the other hand,
%while we can state that $\ell=\ell_1$ for small and large values of $\gamma$ in the case $\tf>1$, %and $\gamma>\gamma_2$,
%for suitable values of $\gamma_1>0$ and $\gamma_2>0$,
it is analytically difficult to infer how the term $\ell_1$ (and hence $\ell$) behaves for $\tf>1$ and generic values of $\gamma$.
%From the facts above and continuity of $\ell_1$ and $\ell_2$,
%we can infer the following result.
%\begin{lemma}\label{lem:bound-deviation}
%	For $\tf=0$,
%	it holds $\ell=\ell_1$.
%	For $\tf>0$,
%	we have $\ell \rightarrow\ell_1^\infty$ as $\gamma\rightarrow0$ and $\ell \rightarrow \ell_2^\infty$ as $\gamma\rightarrow\infty$.
%	Further,
%	by continuity,
%	\eqref{eq:limits-ineq} implies $\ell_1<\ell_2$ for $\gamma<\bar{\gamma}_1$ and $\ell_2<\ell_1$ for $\gamma>\bar{\gamma}_2$,
%	for some finite $\bar{\gamma}_1$ and $\bar{\gamma}_2$ with $\bar{\gamma}_1\le\bar{\gamma}_2$,
%	and the lower bound is $\ell=\ell_1$ for $\gamma<\bar{\gamma}_1$ and $\ell = \ell_2$ for $\gamma>\bar{\gamma}_2$.
%\end{lemma}
%An immediate consequence of~\cref{lem:bound-deviation} is that the bound on deviation due to legitimate agents~\eqref{eq:bound} is strictly decreasing with $\gamma$ if $\tf=0$ and it has a nontrivial minimum point for $\tf>0$.
%On the other hand,
Nonetheless,
the fact (4) above suggests that,
as $\tf$ grows,
$\ell_1$ should have a non-monotonic behavior and admit a nontrivial maximum point.
Indeed,
numerical tests show that $-\ell_1$ is minimized at a finite value of $\gamma$ for every $\tf>1$,
and that such a minimizer decreases as $\tf$ increases,
as illustrated in~\autoref{fig:ell}.
Considering that the bound $\uleg[2]{}$ is proportional to the expectation of $-\ell$,
this further suggests that the deviation decreases for small values of $\gamma$ and increases for large values,
with the minimum point that shifts towards $\gamma=0$ as the more likely values of $\tf$ increase.
This behavior means that, %indeed matches intuition: %consistent with numerical simulations:
%if %$\tf=0$,
%%it means that 
%the legitimate agents immediately identify their adversaries,
%they should ideally remove $\lam{t}$ to follow the standard consensus with learned weights.
%%so that the deviation steadily decreases with $\gamma$.
%Conversely,
%if $\tf>0$,
if the legitimate agents need time to learn which neighbors are trustworthy,
they should act more cautiously and increase the parameter $\lam{t}$,
especially at the beginning.
%where it exhibits a nontrivial minimum point that shifts leftwards as $\tf$ increases.

\begin{figure}
	\centering
	\includegraphics[width=.6\linewidth]{ell}
	\caption{Profile of $-\ell$ in~\eqref{eq:u2} as a function of $\gamma$ with $\tf \in \{2,\dots,10\}$ (the arrow indicates how the curve varies as $\tf$ grows).
		Recall that the bound on (probability of) deviation due to legitimate agents is proportional to $-\mean{\ell}$.
	}
	\label{fig:ell}
\end{figure}

To summarize,
the bound $\uleg[2]{}$ in the deviation term~\eqref{eq:deviation-leg-two-bound}  due to misclassifications of legitimate agents is numerically seen to be quasi-convex with $\gamma$,
with the minimum point that approaches $\gamma=0$ as $\tf$ increases,
\ie according to how difficult learning the true weights $\Wlegtrue$ is.

%Then,
%the final bound reduces to computing the expectation of $\ell$ w.r.t. $\tf$,
%for which we can write upper bounds on the probability.
%In particular,
%the latter bound show that smaller values of $\tf$ are more likely as the confidence in trust scores grows,
%which is consistent with the discussion above.

%By taking the expectation of $\ell$ w.r.t. $\tf$ in~\eqref{eq:w2-ss-bound-exp},
%the bound is a convex combination of all functions $\ell(\gamma;\tf)$,
%and this further suggests that the optimal value of $\gamma$ that minimizes the deviation due to legitimate agents is strictly greater than zero and finite.
%Moreover,
%greater weight is given to the functions with higher probability associated with a specific value of $\tf$.

\begin{comment}
	As for $\Wlegerr[2]{t}$,
	we have
	\begin{equation}\label{eq:leg-err-contribution-lambda-bound}
		\begin{aligned}
			\left|\ls\Wlegerr[2]{t}\stateleg{0}\rs_i\right|	&= \left|\ls\sum_{k=0}^t\lr\prodW{s}{k+1}{t}\rr\lam{k}\stateleg{0}\rs_i\right|\\
			&\stackrel{(i)}{\le} \sum_{k=0}^t\left|\ls\lr\prodW{s}{k+1}{t}\rr\lam{k}\stateleg{0}\rs_i\right|\\
			&\stackrel{(ii)}{\le} \sum_{k=0}^t\lr\prodlam{s}{k+1}{t}\rr\lam{k}\max_{i\in\leg} \left|\ls\stateleg{0}\rs_i\right|\\
			&\stackrel{(iii)}{\le} \eta \sum_{k=0}^t\lr\prodlam{s}{k+1}{t}\rr\lam{k}
		\end{aligned}
	\end{equation}
	where $(i)$ is the triangular inequality,
	$(ii)$ holds because $\Wlegtrue$ is a stochastic matrix,
	and $(iii)$ from $\left|\ls\stateleg{0}\rs_i\right| \le \eta$.
	Then,
	\begin{multline}\label{eq:lambda-series-bound}
		\limsup_{t\rightarrow\infty} \sum_{k=0}^t\lr\prodlam{s}{k+1}{t}\rr\lam{k} \le \sum_{k=0}^\infty (1-\lam{k+1})\lam{k}\\
		=\dfrac{c\e^{-\gamma}\lr\e^\gamma+1-c\rr}{1-\e^{-2\gamma}}.
	\end{multline}
	The bound above is decreasing with $\gamma$ and increasing with $\alpha$.
	This is consistent with the intuition about using $\lam{t}$:
	is $\gamma$ is large,
	then $\lam{t}$ decreases quickly with time and its effect is negligible after a few steps,
	which helps diminishing the deviation if also the true weights are retrieved after a few steps.
	Conversely,
	a small value of $\gamma$ makes the $\lam{t}$'s decay slowly so that the selfishness of agents has non-negligible impact even after the weights have stabilized to the true values.
	The opposite is true as regards $\alpha$:
	large values of $\alpha$ increase the selfishness at all times,
	whereas low values of $\alpha$ induce the agents to rely more on the measurements received from neighbors.
\end{comment}

==> Sections/simulations-old.tex <==
%!TEX ROOT = ../resilient_consensus_trust.tex

\section{Numerical Simulations}\label{sec:simulations}

To test the effectiveness of the proposed resilient consensus protocol and the design insight suggested by the bound proposed in~\cref{thm:bound},
we run numerical simulations with a sparse network with $50$ legitimate agents and $10$ malicious agents.
The communication links are modeled via a random geometric graph with communication radius equal to $0.2$,
the agents being spread across the ball $[0,1] \times [0,1] \in \Real{2}$.
The initial states of legitimate agents are randomly drawn from the uniform distribution $\mathcal{U}(0,\eta)$ with $\eta=1$,
while the malicious agents follow an oscillatory trajectory about the mean value $2\statelegtruess$ (twice the nominal consensus value) under additive zero-mean Gaussian noise with standard deviation $0.05$.
Note that,
in the absence of data-driven detection mechanisms (the malicious agents are classified based on the trust information $\trust{i}{j}{t}$ that comes from physical transmissions and not based on the states they transmit),
this behavior is most harmful because it steadily drives the legitimate agents far away from the nominal consensus value.
Moreover,
it holds $0<2\statelegtruess<1$ and the random oscillations of malicious agents are small compared to their mean value,
which verifies~\cref{ass:initial-state-bound}.

We run the proposed protocol~\eqref{eq:update-rule-regular} with $\lam{t}$ according~\eqref{eq:lambda} with $c=0.9$
for $T=1000$ iterations and average all results across $1000$ Monte Carlo runs.
We report four different setups with different values of $\meanleg$ and $\meanmal$ that respectively increase from $0.55$ to $0.7$ and decrease from $0.45$ to $0.3$.
In all experiments,
the trust observations of legitimate (resp., malicious) transmissions are drawn from the uniform distribution centered at $\meanleg$ (resp., $\meanmal$) with length equal to twice the minimum between $1-\meanleg$ and $\meanmal$.

\begin{figure*}
	\centering
	\includegraphics[width=\linewidth]{Deviation}%
	\hfil
	\includegraphics[width=\linewidth]{Deviation_T1e6}
	\caption{Steady-state deviation from nominal consensus:
		(left) deviation due to legitimate agents $\statelegerr{i}{\infty}$;
        (center) deviation due to malicious agents $\statemalerr{i}{\infty}$;
        (right) total deviation.
        The results are obtained by averaging over $1000$ Monte Carlo runs.
	}
	\label{fig:deviation}
\end{figure*}

The outcomes are depicted in~\autoref{fig:deviation} that shows overall steady-state deviation $\stateerr{i}{\infty}$~\eqref{eq:deviation} in the right box
together with maximal deviation due to legitimate agents $\statelegerr{i}{\infty}$~\eqref{eq:state-leg-error} in the left box
and maximal deviation due to malicious agents $\statemalerr{i}{\infty}$~\eqref{eq:state-mal-error} in the middle box.
It can be seen that the simulated behavior agrees with the analytical bound in~\cref{thm:bound}:
indeed,
the deviation term due to malicious agents steadily increases as $\gamma$ grows,
while the deviation associated with misclassification of legitimate neighbors is minimized by a nonzero value of $\gamma$
that decreases with the uncertainty of trust variables.
For example,
when $\meanleg=0.7$ and $\meanmal=0.3$,
the trust scores are very informative and the deviation is minimized at $\gamma=0.05$,
which dictates a relatively fast decay of the parameter $\lam{t}$.
Conversely,
in the case $\meanleg=0.55$ and $\meanmal=0.45$,
the trust variables are more uncertain and the optimal choice is given by $\gamma=0.01$,
corresponding to a much slower decay of $\lam{t}$.
Moreover,
as the uncertainty in the trust variables increase,
it is more difficult for legitimate agents to correctly classify their neighbors,
which leads to the monotonic increase observed across all deviation terms for every choice of $\gamma$.
